Application of the Space-Time Method to Stimulated Raman Adiabatic Passage on the Simple Harmonic Oscillator

The space-time method is applied to a model system-the Simple Harmonic Oscillator in a laser field to simulate the Stimulated Raman Adiabatic Passage (STIRAP) process. The Space-Time method is a computational theory first introduced by Weatherford et. al. to solve Time-Dependent Systems with one boundary value and applied to electron spin system with invariant Hamiltonian [Journal of Molecular Structure {\bf 592} 47]. The implementation in the present work provides an efficient and general way to solve the Time-Dependent Schr{\"o}dinger Equation and can be applied to multi-state systems. The algorithm for simulating the Simple Harmonic Oscillator STIRAP can be applied to solve STIRAP problems for complex systems.

==> ts_future.tex <==
\section{Future Work}

\label{aaa}

1. Morse ocillator should be tried for multi-level STIRAP process

Although simple harmonic oscillator system can be used to simulate three-level STIRAP process, it is not good for multi-level STIRAP process. In a simple harmonic oscillator system, the relation of energy differences between nearby levels, $E_{j+1} - E_j= E_j-E_{j-1}$, holds for every $j$. Thus, if simple harmonic oscillator system is used to simulate a multi-level STIRAP process, the pump pulse frequency $\omega_p=\frac{E_1-E_0}{\hbar}$ and the Stokes pulse frequency $\omega_s=\frac{E_n-E_{n-1}}{\hbar}$ have same value $\omega_0$, then these pulse coherent with every nearby level pairs and stimulated population transfer from one energy level to its neighbor below level happens. It is very hard to transfer large population to the target state.

In a Morse ocillator system, the energy differences between nearby levels are not the same. An external laser pulse will not coherent with every nearby state pair. It is expected to simulate multi-level STIRAP process for a Morse oscillator.

One thing needs to be concerned is the dipole moment. For Morse oscillator,
$\langle j \vert  r \vert j+2 \rangle \neq 0$. While for a ideal STIRAP process,
$\langle j \vert  r \vert j+2 \rangle = 0$ is required.


2. Optimal control for STIRAP

A basic assumption and have been used in our calculation is that the integration of effective Rabi frequency is $\pi$. This can be applied to the optimal control for STIRAP process as a constraint, and better result is expected. In \cite{ISOLAPRA60}, the energy fluecy of the fields, $\sum_n \int_0^T \mathrm{d} t \Omega_n^2(t)$, is introduced but not used in calculation. The $\pi$ integration should be applied for this kind of constraints. 


2.1 For two pulses STIRAP process, the effective Rabi frequency is known. If the above $\pi$ integral constraint is applied to the optimal control process, higher population transfer should be obtained compare with the results in \cite{ISOLAPRA60}.

2.2 For multi-level STIRAP process, I am not sure about the effective Rabi frequency and what the contraints looks like. I need consider this problem and try to find out the effective Rabi frequency and the constraint for the pulses which connnecting the intermediate levels.

I will do 1 first, then 2.1, then 2.2.



==> ts_gauss_stirap.tex <==
\subsection{Stimulated Raman Adiabatic Passage with Gauss-Shape Laser Field}
\label{subsec:PGAUSS}

\begin{figure}
\includegraphics[width=.8500\columnwidth]{cj_sho3lgausssumprb}
\caption[]
{(color online) Target state population vs. the variance of Gauss pulse for defferent pulse delay in STIRAP process for a simple harmonic oscillator in Gauss pulse laser field. Here $\Omega_s \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_s)^2/(2\sigma^2)}$,$\Omega_p \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_p)^2/(2\sigma^2)}.$}
\label{cj_sho3lgausssumprb}
\end{figure}

Now we consider a simple harmonic oscillator system with ground state and the first two excited states in a Gauss pulse laser field. For simplicity, the pump pulse width (the variance) and the Stokes pulse width are set to be the same ($\sigma$); the peak point of the Stokes pulse ($\tau_s$) and the peak point of the pump pulse ($\tau_p$) are set to be symmetric about the mid-point of the whole external field length. The pulse delay is $\Delta\tau=\tau_p-\tau_s$. Thus, the pulse shape functions $s \left(t\right)$ and $p\left(t\right)$ can be written as,

\begin{eqnarray}
s \left( t \right) &=& \frac{1}{\sigma \sqrt{2 \pi}}e^{-\frac{(t-\tau_s)^2}{2\sigma^2}},\\
p \left( t \right) &=& \frac{1}{\sigma \sqrt{2 \pi}}e^{-\frac{(t-\tau_p)^2}{2\sigma^2}}.
\end{eqnarray}


Then the Rabi requencies for the Stokes and pump pulses are,

\begin{eqnarray}
\Omega_s \left( t \right) &=&A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-\frac{(t-\tau_s)^2}{2\sigma^2}},\\
\Omega_p \left( t \right) &=&A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-\frac{(t-\tau_p)^2}{2\sigma^2}}.
\end{eqnarray}

\begin{figure}
\includegraphics[width=.8500\columnwidth]{cj_sho3lgausssumprbpart}
\caption[]
{(color online) Target state population vs. the variance of Gauss pulse for defferent pulse delay in STIRAP process for a simple harmonic oscillator in Gauss pulse laser field. Only the neighbor part of the maximum populations is shown. The maximum value shown in the figure is from our calculation. Due to the random chosen of pulse delay $\Delta\tau$ and pulse width $\sigma$, the value of maximum population $0.88889175$ and the corresponding pulse delay $\Delta\tau=0.9 \times 10^6$, the pulse width $1.4 \times 10^6$ may not be correct and accurate.}
\label{cj_sho3lgausssumprbpart}
\end{figure}

We calculate the STIRAP process with different pulse variances and different time delays. In our calculation, the pulse delay $\Delta\tau$ varies from $0.7 \times 10^6$ to $1.6 \times 10^6$. For small pulse delays, $\Delta\tau=0.7 \sim 1.0 \times 10^6$, the pulse width varies from $1.0 \times 10^6$ to more than $3.0 \times 10^6$, while for large pulse delays, $\Delta\tau=1.1 \sim 1.6 \times 10^6$, the pulse width varies from $1.55 \times 10^6$ to more than $3.0 \times 10^6$. Fig.~(\ref{cj_sho3lgausssumprb} shows the target state population vs. pulse variance curves for different pulse delays. From the plot, we can see that the population transfer to the target state is related to the pulse variance $\sigma$ and pulse delay $\Delta\tau$. From the plot, it can be seen that for the same pulse delay, the population in the target state increases as the variance increases and then goes down slowly after it reaches a maximum value. The maximum value of the population in the target state for each time delay is larger than $0.88$ although the maximum points for different pulse delays are with different pulse widths (variance). While the pulse delay $\Delta\tau$ increase from $0.7 \times 10^6$ to $1.6 \times 10^6$, the pulse widths ( the pulse variance, $\sigma$) which leads to the maximum population transfer to the target state moves from $1.55 \times 10^6$ to $2.25 \times 10^6$.   


\begin{figure}
\includegraphics[width=.8500\columnwidth]{cj_sho3lgausslaser}
\caption[]
{(color online) Laser pulse in STIRAP for a simple harmonic oscillator in laser field. Here $\Omega_s \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_s)^2/(2\sigma^2)}$,$\Omega_p \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_p)^2/(2\sigma^2)}.$}
\label{cj_sho3lgausslaser}
\end{figure}

\newpage
\begin{figure}
\includegraphics[width=.8500\columnwidth]{cj_sho3lgaussomega}
\caption[]
{(color online) Rabi frequencies in STIRAP procession for simple harmonic oscillator in laser field. Here $\Omega_s \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_s)^2/(2\sigma^2)}$,
$\Omega_p \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_p)^2/(2\sigma^2)}.$}
\label{cj_sho3lgaussomega}
\end{figure}

Fig.~(\ref{cj_sho3lgausssumprbpart}) is part of Fig.~(\ref{cj_sho3lgausssumprb}) in which only the neighbor part of the maximum populations is shown. From our calculating result, we obtained maximum target population $0.88889175$, which corresponds to pulse delay $\Delta\tau = 0.9 \times 10^6$ and pulse width $\sigma=1.4 \times 10^6$. Although this result is good enough to reflect the relationship between the population transfer and the pulse shap functions, calculation for more values of  pulse delay $\Delta\tau$ and pulse width $\sigma$ is needed to get more accurate values. 

\begin{figure}
\includegraphics[width=.8500\columnwidth]{cj_sho3lgaussprb}
\caption[]
{(color online) Population transfer in STIRAP procession for simple harmonic oscillator in laser field. Here $\Omega_s \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_s)^2/(2\sigma^2)}$,
$\Omega_p \left( t \right) =A_0 \frac{1}{\sigma \sqrt{2 \pi}}e^{-(t-\tau_p)^2/(2\sigma^2)}.$
}
\label{fig:cj_sho3lgaussprb}
\end{figure}

Fig.~(\ref{cj_sho3lgausslaser}), Fig.~(\ref{cj_sho3lgaussomega}) and Fig.~(\ref{fig:cj_sho3lgaussprb}) show the plots for the external laser field, the Rabi frequency, and population transfer. In these plots, the pulse delay is $\Delta\tau=0.9 \times 10^6$ and the pulse width is $\sigma=1.4 \times 10^6$, which are the maximum values from our calculation.

